Power Operations in Morava E-Theory of Flat Ring Spectra

Let $E_n$ be Morava $E$-theory of height $n$. Let $R$ be a $p$-adically flat commutative ring spectrum. Then the Tate-valued Frobenius map endows $\pi_0 R$ with the structure of a $\delta$-ring. On the other hand, we may form the $K(n)$-completed tensor product $L_{K(n)}(R \otimes E_n)$, which is a $K(n)$-local $E_n$-algebra. Then $\pi_0(L_{K(n)}(R \otimes E_n)) = LT_n \widehat{\otimes} \pi_0 R$ admits the structure of an algebra over the monad $\mathbb{T}(n)$ defined by Rezk. The $\mathbb{T}(n)$-algebra structure encodes the power operations of $L_{K(n)}(R \otimes E_n)$. In this paper we describe the $\mathbb{T}(n)$-algebra structure on $\pi_0(L_{K(n)}(R \otimes E_n))$.

==> macro.tex <==
\ProvidesPackage{ekzhang}

\usepackage{amsmath,amsfonts,amssymb,amsthm}
\usepackage{asymptote}
\usepackage{cancel}
\usepackage{color}
\usepackage[dvipsnames]{xcolor}
\usepackage{enumerate}
\usepackage{graphicx}
\usepackage{mathtools}
\usepackage{minted}
\usepackage{tikz,tikz-cd}
\usepackage{verbatim}
\usepackage[dvipsnames]{xcolor}

\usepackage{thmtools}

\usepackage[a4paper, left=3cm, right=3cm, top=3cm, bottom=4cm]{geometry}

\usepackage[colorlinks=true]{hyperref}
\hypersetup{
    linkcolor=NavyBlue,
    citecolor=ForestGreen,
    filecolor=Plum,
    urlcolor=RubineRed,
}
\usepackage[capitalise,nameinlink]{cleveref}

\theoremstyle{definition}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lem}[thm]{Lemma}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{definition}[thm]{Definition}
\newtheorem{construction}[thm]{Construction}
\newtheorem{example}[thm]{Example}

\newtheorem{blah}{Theorem}

\newtheorem*{note}{Note}
\newtheorem*{claim}{Claim}

\theoremstyle{remark}
\newtheorem{rmrk}[thm]{Remark}


\crefname{cor}{Corollary}{Corollaries}
\crefname{lem}{Lemma}{Lemmas}
\crefname{prop}{Proposition}{{Propositions}}

\newcommand{\AAA}{\mathbb{A}}
\newcommand{\BB}{\mathbb{B}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\FF}{\mathbb{F}}
\newcommand{\GG}{\mathbb{G}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\II}{\mathbb{I}}
\newcommand{\JJ}{\mathbb{J}}
\newcommand{\KK}{\mathbb{K}}
\newcommand{\LL}{\mathbb{L}}
\newcommand{\MM}{\mathbb{M}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\OO}{\mathbb{O}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\UU}{\mathbb{U}}
\newcommand{\VV}{\mathbb{V}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}}

\newcommand{\scA}{\mathcal{A}}
\newcommand{\scB}{\mathcal{B}}
\newcommand{\scC}{\mathcal{C}}
\newcommand{\scD}{\mathcal{D}}
\newcommand{\scE}{\mathcal{E}}
\newcommand{\scF}{\mathcal{F}}
\newcommand{\scG}{\mathcal{G}}
\newcommand{\scH}{\mathcal{H}}
\newcommand{\scI}{\mathcal{I}}
\newcommand{\scJ}{\mathcal{J}}
\newcommand{\scK}{\mathcal{K}}
\newcommand{\scL}{\mathcal{L}}
\newcommand{\scM}{\mathcal{M}}
\newcommand{\scN}{\mathcal{N}}
\newcommand{\scO}{\mathcal{O}}
\newcommand{\scP}{\mathcal{P}}
\newcommand{\scQ}{\mathcal{Q}}
\newcommand{\scR}{\mathcal{R}}
\newcommand{\scS}{\mathcal{S}}
\newcommand{\scT}{\mathcal{T}}
\newcommand{\scU}{\mathcal{U}}
\newcommand{\scV}{\mathcal{V}}
\newcommand{\scW}{\mathcal{W}}
\newcommand{\scX}{\mathcal{X}}
\newcommand{\scY}{\mathcal{Y}}
\newcommand{\scZ}{\mathcal{Z}}

\DeclarePairedDelimiter{\pa}{\lparen}{\rparen}
\DeclarePairedDelimiter{\br}{[}{]}
\DeclarePairedDelimiter{\cbr}{\{}{\}}
\DeclarePairedDelimiter{\ang}{\langle}{\rangle}
\DeclarePairedDelimiter{\abs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\dabs}{\|}{\|}
\DeclarePairedDelimiter{\eval}{.}{|}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}

\newcommand{\p}{\partial}
\newcommand{\dd}{\mathop{}\!\mathrm{d}}
\newcommand{\dv}[3][]{\frac{\dd^{#1} #2}{\dd #3^{#1}}}
\newcommand{\pdv}[3][]{\frac{\p^{#1} #2}{\p #3^{#1}}}
\newcommand{\del}{\nabla}
\newcommand{\phii}{\varphi}


\newcommand{\mat}[1]{\begin{matrix} #1 \end{matrix}}
\newcommand{\smat}[1]{\begin{smallmatrix} #1 \end{smallmatrix}}
\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\bsmat}[1]{\begin{bsmallmatrix} #1 \end{bsmallmatrix}}
\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}
\newcommand{\psmat}[1]{\begin{psmallmatrix} #1 \end{psmallmatrix}}

\newcommand{\E}[1]{\operatorname{\mathbf{E}}\left[#1\right]}
\newcommand{\Var}[1]{\operatorname{\mathbf{Var}}\left[#1\right]}

\newcommand{\lcm}{\operatorname*{lcm}}
\newcommand{\argmax}{\operatorname*{arg max}}
\newcommand{\argmin}{\operatorname*{arg min}}


\newcommand{\into}{\hookrightarrow}
\newcommand{\onto}{\twoheadrightarrow}

\newcommand{\RP}{\mathbb{RP}}
\newcommand{\CP}{\mathbb{CP}}

\newcommand{\im}{\operatorname{Im}}
\newcommand{\rank}{\operatorname{rank}}
\newcommand{\ch}{\operatorname{char}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\Id}{\operatorname{Id}}
\newcommand{\Cone}{\operatorname{Cone}}
\newcommand{\ord}{\operatorname{ord}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\Aut}{\operatorname{Aut}}
\newcommand{\Pic}{\operatorname{Pic}}
\newcommand{\Ann}{\operatorname{Ann}}
\newcommand{\Sym}{\operatorname{Sym}}
\newcommand{\Frac}{\operatorname{Frac}}
\newcommand{\GL}{\operatorname{GL}}
\newcommand{\SL}{\operatorname{SL}}
\newcommand{\Ob}{\mathrm{Ob}}
\newcommand{\Mor}{\mathrm{Mor}}
\newcommand{\spec}{\mathrm{spec}}
\newcommand{\proj}{\mathrm{proj}}
\newcommand{\Alg}{\mathrm{Alg}}
\newcommand{\ev}{\mathrm{ev}}
\newcommand{\Spec}{\mathrm{Spec}}
\newcommand{\Sky}{\mathrm{Sky}}
\newcommand{\spann}{\mathrm{span}}
\newcommand{\rk}{\mathrm{rk}}

\newcommand{\frakp}{\mathfrak{p}}

\newcommand{\eps}{\varepsilon}
\newcommand{\frakm}{\mathfrak{m}}
\newcommand{\fraka}{\mathfrak{a}}

\newcommand{\ds}{\displaystyle}
\newcommand{\on}{\operatorname}
\newcommand{\nc}{\newcommand}

\newcommand{\colim}{\operatorname{colim}}
\newcommand{\Ext}{\operatorname{Ext}}
\newcommand{\Spf}{\operatorname{Spf}}
\newcommand{\cofib}{\operatorname{cofib}}
\newcommand{\Frob}{\operatorname{Frob}}
\newcommand{\Def}{\operatorname{Def}}
\newcommand{\op}{\operatorname{op}}
\newcommand{\Cat}{\operatorname{Cat}}
\newcommand{\Mod}{\operatorname{Mod}}
\newcommand{\Sh}{\operatorname{Sh}}
\newcommand{\CAlg}{\operatorname{CAlg}}

\newcommand{\Fun}{\operatorname{Fun}}
\newcommand{\Sp}{\operatorname{Sp}}

\newcommand{\ho}{\operatorname{ho}}

\newcommand{\tr}{\operatorname{tr}}
\newcommand{\can}{\operatorname{can}}

\usepackage{xparse}

\NewDocumentCommand{\cotimes}{o}{%
    \,\widehat{\otimes}\IfValueT{#1}{_{#1}}\,%
}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

\newcommand{\Tor}{\operatorname{Tor}}
\newcommand{\Orb}{\operatorname{Orb}}
\newcommand{\free}{\text{free}}

\newcommand{\pcs}{\SSS_{p}^{\wedge}}

\newcommand{\Mon}{\mathrm{Mon}}
\newcommand{\Level}{\mathrm{Level}}
\newcommand{\Type}{\mathrm{Type}}
\newcommand{\Sub}{\mathrm{Sub}}
\newcommand{\rest}{\mathrm{rest}}

\newcommand{\Div}{\mathrm{Div}}




\newcommand{\red}[1] {\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\purple}[1]{\textcolor{purple}{#1}}
\newcommand{\pink}[1]{\textcolor{Mulberry}{#1}}

\newcommand{\yuval}[1]{\purple{Yuval: #1}}
\newcommand{\shachar}[1]{{\red{Shachar: #1}}}
\newcommand{\noam}[1]{\pink{Noam: #1}}

